Error analysis of a demodulation procedure for multicarrier signals with slowly-varying carriers

We propose a procedure to demodulate analog signals encoded by a multicarrier modulator, with slowly-varying carrier shapes. We prove that the asymptotic demodulation error can be made arbitrarily small. The intended application is the "sensorless" control of AC electric motors at or near standstill, through the decoding of the PWM-induced current ripple.

==> proof_k.tex <==
\section{Appendix: proof at any order}
\subsection{Theorem}
In this subsection, we prove that for the kth-order moving average kernel $\varphi_k$, we have $\varphi_k * s_0 = O(\varepsilon^k)$. 
\subsection{For a general kernel}
The next result holds for any regular-enough kernel $\varphi$ and provides a general expression for the convolution of $\varphi$ with a carrier $s(t,\tfrac{t}{\varepsilon})$. 
\begin{theorem}
	Let $\varphi \in C^k$. Then 
	\begin{equation}
		\varphi *  s_0 =(-\varepsilon)^k \sum_{i=0}^k (-1)^i \binom{k}{i} \varphi^{(i)} * \partial_1^{k-i}  s_k. 
		\label{eq:phi_star_s0}
	\end{equation}
	\label{th:estimate}
\end{theorem}

\begin{proof}
	This result is proved by induction. It is immediately satisfied for $k=0$. For $k \to k+1$, we use the identity $\frac{d}{d\sigma} \partial_1^{k-i} s_{k+1} = \partial_1^{k-i+1} s_{k+1} + \frac{1}{\varepsilon} \partial_1^{k-i} s_k$ for $0 \leq i \leq k$ so that the terms in the sum~\eqref{eq:phi_star_s0} read
\begin{align}
	\varphi^{(i)} * \partial_1^{k-i}  s_k = \varepsilon \varphi^{(i)} * (\frac{d}{d\sigma} \partial^{k-i} s_{k+1} - \partial_1^{k-i+1} s_{k+1}). 
	\label{eq:proof_phi_star_part}
\end{align}
Using the properties of the convolution product, the first term of~\eqref{eq:proof_phi_star_part} is simply
\begin{align*}
	\varphi^{(i)} * \frac{d}{d\sigma} \partial_1^{k-i}  s_{k+1} = \varphi^{(i+1)} * \partial_1^{k-i}  s_{k+1}. 
\end{align*}
Thus, replacing every terms of~\eqref{eq:phi_star_s0} by ~\eqref{eq:proof_phi_star_part} yields
\begin{IEEEeqnarray*}{rCl}
	\varphi *  s_0 &=& \, (-\varepsilon)^k \varepsilon \sum_{i=0}^k (-1)^i \binom{k}{i} \varphi^{(i+1)} * \partial_1^{k-i}  s_{k+1} \\
		       &&\, + (- \varepsilon)^{k+1}\sum_{i=0}^k (-1)^i \binom{k}{i} \varphi^{(i)} * \partial_1^{k-i+1}  s_{k+1} \\
		       &=& \, (-\varepsilon)^{k+1} \sum_{i=1}^{k+1} (-1)^{i} \binom{k}{i-1} \varphi^{(i)} * \partial_1^{k+1-i}  s_{k+1} \\
	 &&\, (-\varepsilon)^{k+1}+ \sum_{i=0}^k (-1)^{i}\binom{k}{i} \varphi^{(i)} * \partial^{k+1-i}_1  s_{k+1}\\
	 &=& (-\varepsilon)^{k+1} \sum_{i=0}^{k+1}(-1)^i \binom{k+1}{i} \varphi^{(i)} * \partial^{k-i}_1  s_{k+1}
\end{IEEEeqnarray*}
by Pascal's rule. 
\end{proof}

For a kernel $\varphi$ with compact support $K$, with $l(K) := \int 1_K$, 
\begin{align*}
	\| \varphi *  s_0 \|_\infty \leq \varepsilon^k \sum_{i=0}^k \binom{k}{i} l(K) \|\varphi^{(i)} \|_\infty \|\partial_1^{k-i}  s_k \|_\infty
\end{align*}
This estimate is nonetheless not enough to prove $\varphi_k * s_0 = O(\varepsilon^k)$ for the moving average kernels with a window length of $\varepsilon$ since $l(K) = k\varepsilon $ but $\| \varphi_k^{(i)} \|_\infty = O(1/\varepsilon^{1+i})$. However, we can still refine the estimate for this particular kernel. 

\subsection{For the moving-average kernel}

\begin{theorem}
	Let $\zeta_{i}(\upsilon,\sigma)$ $C^{i}$ and $C^{i+1}$ by part with zero mean in $\sigma$ for fixed $\upsilon$,  such that $\zeta_{i+j}$, the zero-mean primitive in $\sigma$ of $\zeta_{i+j}$ is $C^{i+j}$ and $C^{i+j+1}$ by part. Then 
	\begin{align*}
		\varphi_k^{(k-i)} * \zeta_{k-i} = O(\varepsilon^i)
	\end{align*}
\end{theorem}

\begin{proof}
	(Reminder: $\varphi_k^{(j)} = O(\frac{1}{\varepsilon^{1+j}})$)
	By induction. For $i = 0$, by lemma 2
	\begin{align*}
		\varphi_k^{(k)} *  \zeta_k = \frac{1}{\varepsilon^k} \Delta_k   \zeta_k = O(1)
	\end{align*}
Assume the estimate holds for $i$. 
\begin{align*}
	\varphi_k^{(k-i-1)}  \zeta_{k-i-1} &= \varepsilon \varphi_k^{(k-i)} * \zeta_{k-i} - \varepsilon \varphi_k^{(k-i-1)} * \partial_1  \zeta_{k-i} \\
					 &= \sum_{j=0}^N (-1)^j \varepsilon^{j+1} \varphi_k^{(k-i)} * \partial_1^j  \zeta_{k-i+j}  \\
					 & -(-\varepsilon)^N \varphi_k^{(k-i-1)}*\partial_1^{N+1}  \zeta_{k-i+N}
\end{align*}
Since $\| \varphi_k^{(k-i-1)} \|_\infty = O(1/\varepsilon^{k-i})$, we choose $N = k+1$ so that 
\begin{align*}
	\varepsilon^N \varphi_k^{k-i-1} * \partial_1^{N+1}   \zeta_{k-i+N}  =  O(\varepsilon^{i+1}), 
\end{align*}
and for $0 \leq j \leq N$, by hypothesis,
\begin{align*}
	\varepsilon^{j+1} \varphi_k^{k-i} * \partial_1^j  \zeta_{k-i+j} = O(\varepsilon^{i+1})
\end{align*}
\end{proof}
We finally use this result on the expression for $\varphi *  s_0$ 



==> proof_with_integrals.tex <==
\begin{IEEEeqnarray*}{rCl}
	(K_3 * s)(t) &:=& \int_{t-t_k}^t K_3(t-\sigma) s(\sigma,\tfrac{\sigma}{\varepsilon}) \, d\sigma \\
		     &=& \varepsilon \int_{t-t_k}^t K_3(t-\sigma) (\frac{d}{d\sigma} s^{-1} (\sigma,\tfrac{\sigma}{\varepsilon})  - \partial_1 s^{-1}(\sigma,\tfrac{\sigma}{\varepsilon}))  \, d\sigma \\
		     &=& \varepsilon [K_3(t-\sigma)s^{-1}(\sigma,\tfrac{\sigma}{\varepsilon}) ]^t_{t-t_k}  \\
		     &&\, + \varepsilon \int_{t-t_k}^t K_3'(t-\sigma) s^{-1} (\sigma,\tfrac{\sigma}{\varepsilon}) \, d\sigma \\
		     &&\, - \varepsilon \int_{t-t_k}^t K_3(t-\sigma) \partial_1 s^{-1} (\sigma,\tfrac{\sigma}{\varepsilon}) \, d\sigma
\end{IEEEeqnarray*}
The first term is zero since $K_3(0) = K_3(t_k) = 0$. And the last term shares the same form as $K_3 * s$. Repeating the same computation on the first integral using the identity $\frac{ds^{-2}}{d\sigma} = \partial_1 s^{-2} + \frac{1}{\varepsilon} s^{-1}$, $\varepsilon K_3' * s^{-1}$ reads
\begin{IEEEeqnarray*}{rCl}
	\varepsilon \int_{t-t_k}^t K_3'(t-\sigma) s^{-1} \, d\sigma &=& \varepsilon^2 [K_3'(t-\sigma)s^{-2} ]^t_{t-t_k}  \\
								    &&\hspace{-9em}+ \varepsilon^2 \int_{t-t_k}^t K_3''(t-\sigma) s^{-2}
		      - \varepsilon^2 \int_{t-t_k}^t K_3'(t-\sigma) \partial_1 s^{-2} d\sigma.
\end{IEEEeqnarray*}
The first term is zero since $K_3'(0) = K_3'(t_k) = 0$. 

And the last term shares the same form as $K_3' * s^{-1}$.

